Examining Political Rhetoric with Epistemic Stance Detection

Participants in political discourse employ rhetorical strategies -- such as hedging, attributions, or denials -- to display varying degrees of belief commitments to claims proposed by themselves or others. Traditionally, political scientists have studied these epistemic phenomena through labor-intensive manual content analysis. We propose to help automate such work through epistemic stance prediction, drawn from research in computational semantics, to distinguish at the clausal level what is asserted, denied, or only ambivalently suggested by the author or other mentioned entities (belief holders). We first develop a simple RoBERTa-based model for multi-source stance predictions that outperforms more complex state-of-the-art modeling. Then we demonstrate its novel application to political science by conducting a large-scale analysis of the Mass Market Manifestos corpus of U.S. political opinion books, where we characterize trends in cited belief holders -- respected allies and opposed bogeymen -- across U.S. political ideologies.

==> files/DataCollection.tex <==
% !TEX root = ../main.tex

\section{Data Collection}
\label{sec:data_collection}
We sample sentences for annotation from 308 political books drawn from \emph{Contemporary American Ideological Books Corpus} (CAIB; \citealp{sim2013measuring}), a collection of mass-market political nonfiction books written by contemporary U.S.\ political figures such as national politicians, media personalities, and advocates.

For collecting epistemic stance annotations, we sampled one sentence per book. To ensure a dataset with a range of complex linguistic and rhetorical phenomena, we considered sentences with more than 15 tokens and at least one embedded event clause, defined as follows.
%(see Events and Sources below).
 \jhg{Did you do any filtering to get sentences that involved political rhetoric? Or did you randomly choose a single sentence without any filtering or chance for rejection (e.g. if sentence were simply the author recalling trips to Lake Erie as a child).}
%As a result, we collected 91,343 judgments for 9,867 (before quality filtering; see below) event-source pairs (on average 9.25 judgments per pair). \scomment{do we even need this statistic?}

\textbf{Events and Sources}\ \ 
In order to annotate sentences from the corpus, we must first identify, for each sentence, relevant events and sources to analyze.
Our approach is to over-generate, identifying many possible events and sources, and rely on non-epistemic annotations and their modeling to identify instances of meaningful epistemic stances.

%We take an approach oriented toward how a factuality analyzer would be realistically run on a new corpus.
While we use \factbank's framing of the semantic analysis problem, we find its approach to event-source identification problematic. \factbank identifies its event tokens as the ones marked in the highly precise, manually annotated \timebank and AQUAINT TimeML\footnote{\url{http://www.timeml.org/site/timebank/timebank.html}} corpora, but to analyze epistemic stances in raw text, events must of course be automatically identified.

By contrast, we seek to identify all heads of sentential clauses as events. With an automatic parser with Universal Dependencies (v1.3) formalism~\cite{NIVRE16.348}\footnote{CoreNLP 3.8.0 with its `english\_UD' pretrained model} \bto{UD version, what software parser and version? and proper citation.}, we designate the tree's
root as an event, as well as its descendants connected via any of the relations \emph{acl:relcl, advcl, ccomp, csubj, parataxis, xcomp}.\footnote{This heuristic has the limitation of excluding nominal events, such as \emph{The \textbf{firing} of the manager}, which is beyond the purview of this project.} 
% In contrast with ours, FactBank draws its events from a highly precise, manually annotated Timebank and AQUAINT TimeML corpus.

Finding sources also presents a challenge. 
\factbank only analyzes sources that are subjects of
% requires sources to be introduced by
\emph{source-introducing predicates} (SIPs), from a lexicon of verbs about report and belief, such as \emph{claim, doubt, feel, know, say, think} \cite{sauri2012you}.
% the subjects of these predicates are taken to be sources. For example, in a sentence such as ``Jane thinks that Sarah went to the party", the SIP \emph{thinks} introduces the source \emph{Jane}. 
However, this can miss potentially relevant sources.
% not introduced predicates not in the lexicon, as in:
% \emph{Yesterday [Congress]$_{\text{s1}}$ \textbf{passed}$_{\text{e1}}$ the bill.}
% \bto{not a great example - not meaningful for our ultimate goal} In this example, we prefer to predict that \emph{Congress} has a factuality stance towards the bill's passage, and in general, we treat any entity (named or otherwise) that could be reasonably regarded to have an opinion about an event as a source. 
Therefore, we use a loose automatic filter that considers all nouns or pronouns (that do not have a noun or adjective parent) as a source.  The special \emph{Author} source is always included as a source. We also simplified \factbank's source selection process by excluding nested sources\footnote{}. For a vast majority of sentences in our corpus, nested sources seemed not to be necessary. Furthermore, it was challenging to train crowd-workers to interpret stances for nested sources.

Finally, we consider the cross-product of all pairs of sources and events within a sentence, asking annotators to give a stance value for each pair.  This can lead to a large number of tuples, especially in longer sentences, and it over-generates spurious candidate pairs, which makes necessary the common \nonepistemic~label. We believe this over-generation, however, helps give a realistic evaluation of multi-source epistemic stance analysis on a new corpus.

\textbf{Annotation Process}
We conducted an initial pilot study with 19 sentences, attempting to delineate a reporting stance (where a source reports what someone else has said, without taking a stance whether it happened) versus a general uncommitted stance, following \citealp{prabhakaran2015new} who annotated for reported beliefs; however, we found annotators often confused them for one another, so we merged them. %\bto{su lin: is my reporting stance defin correct and can it be shorter?} \bto{this text said Diab 2009 did reporting, but actually they included it within a very broad uncommitted/neg class}
We proceeded to the larger scale annotation; a sample prompt is shown in Appendix's Figure~\ref{fig:prompt}.
After the additional quality control filtering described below, we obtain a raw inter-annotator agreement rate $0.793$ and chance-adjusted agreement rate (Krippendorff $\alpha$) $0.554$ for 51,805 annotations. 
% Table~\ref{tab:cmm} provides the conditional confusion matrix for each label using raw annotations for each item, the diagonal entries showing annotator agreement for each class. Annotators mostly agree for all classes except for the uncommitted classes, where the agreement rate is slightly lower; we examine this further in Section~\ref{sec:mace}. 
%We elaborate more on this in Section~\ref{sec:mace}, where we show that the annotators find such items difficult and have inherent subjective opinion about the factuality of these items, often confusing between positive/negative versus uncommitted. 
This is broadly in line with reported chance-adjusted agreement rates for author-only factuality annotations: $0.60$ in \citet{prabhakaran2015new} or $0.66$ in \citet{rudinger2018neural}. For multi-source factuality annotations, \citet{sauri2012you} reported an overall chance-adjusted agreement rate of 0.81, however it only covers 30$\%$ of all the events in the corpus; \citet{de-marneffe-etal-2012-happen} reports an agreement rate of $0.66$ for the three-category (positive, negative, Uu) version of their factuality annotations from reader's perspective, with the agreement rate for 7 class fine-grained categorization being even lower.  
\bto{todo discuss s+p and marneffe which are a lot higher, wtf?}
While agreement rate for our dataset is slightly lower than some of the conventional standards seen in NLP, this task has genuine, substantive ambiguity, which could be captured and analyzed in future work along the lines of \citet{pavlick2019inherent}'s study of natural language inference.

%\textbf{Resources Utilized}\ \ 
Annotations were collected on the Figure Eight platform.\footnote{Annotation costs were supported by [removed for anonymity].
%a Figure Eight ``AI for Everyone Challenge'' grant.
} Crowdworkers were selected from the highest contributor level (level 3) and were limited to those from the US; we did not limit to native English speakers.
Workers were paid \$0.10 per annotation, with a median 54 (mean 115) seconds per annotation. Worker speeds varied by multiple orders of magnitude (from 1.8 to 355 sec/anno, averaged per worker).
%   \scomment{payment? definitely a part of ethical review now}
%   \bto{i once computed the hourly wage histogram and it was log-normal like all these things are. imo research/industry standards havent caught up to where it's feasible to do ethical review}
% In total, the 
% main annotations took nine days (from 11/28/2018 to 12/09/2018) to complete,
% costing approximately \$11,000.

We used three strategies, each of which we observed improved data quality.
(1) During annotation, we used Figure Eight's ``hidden gold'' testing facility to restrict to workers who had a high agreement rate with a number of tuples from \factbank which we designated as a gold standard. \scomment{is there any risk that there might be meaningful dissensus on these items?}
(2) We removed judgments originating from IP addresses used by more than one unique worker, or from workers associated with more than five IP addresses, which seemed to be low quality annotations. 
(3) After discarding items with fewer than three judgments, we infer final aggregated labels via the MACE model and software \cite{hovy2013learning},\footnote{\url{https://github.com/dirkhovy/MACE}}
which uses Bayesian unsupervised learning to weigh the judgments of different annotators by their relative reliability;
\citet{Paun2018Comparing} found MACE was one of the best models for crowdsourced annotation aggregation. We consider the most probable label inferred by MACE to be the final label in our corpus.  
%The appendix (Table~\ref{table:disagreement}) shows high-disagreement examples identified from high posterior label entropy.

%, as determined through Bayesian unsupervised learning.
%\textbf{Amount of Data}\ \ 
After quality filtering, our dataset consists of 8465 event-source pairs spanning 308 sentences from the CAIB corpus (Table~\ref{table:stats}).

% \begin{table}[]
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\#Sentences} & \multicolumn{5}{c|}{\#Event-Source Tuples}   \\ \cline{2-6} 
%                              & Total & Pos  & Neg & Uu  & NE   \\ \hline
% \multicolumn{1}{|c|}{308}    & 8465  & 1176 & 254 & 641 & 6394 \\ \hline
% \end{tabular}
% \caption{\polibelief corpus statistics; Pos: positive, Neg: negative, Uu: uncommitted, NE: non-epistemic}
% \label{table:stats}
% \end{table}


\begin{table}[]
\begin{tabular}{c|rrrrr}
\hline \addlinespace[0.05cm]
\multirow{2}{*}{\#Sentences} & \multicolumn{5}{c}{\#Tuples}    \\ \addlinespace[0.05cm] \cline{2-6}  \addlinespace[0.05cm]
                             & Pos  & Neg & Uu  & NE   & Total \\ \addlinespace[0.05cm] \hline \addlinespace[0.05cm]
\multicolumn{1}{r|}{308}     & 1176 & 254 & 641 & 6394 & 8465  \\ \addlinespace[0.05cm] \hline \addlinespace[0.05cm]
\end{tabular}
\caption{\polibelief corpus statistics; Pos: positive, Neg: negative, Uu: uncommitted, NE: non-epistemic}
\label{table:stats}
\end{table}



%Unlike FactBank, we choose to follow coarse grained annotation framework as it supports our semantic application requirements and is easy for crowd source workers. Too many classes often confuse these workers resulting in low agreement rates. Our application requires us to include ``non-epistemic" class. FactBank assumes that the legitimate events and sources are pre-defined. However, for factuality analysis on political books, we don't even know what are legitimate events and sources. Thus, we are taking a semantic edge parsing/relational parsing approach. Predicting ``non-epistemic" class is like lack of factuality edge. Similar to SRL or semantic dependency parsing task prominent in current literature~\cite{oepen-etal-2014-semeval}, we annotate events and sources at token level. 

% \textbf{FB versus Polibelief data qualitative analysis}
% Table 2 shows some statistical descriptions of the two datasets. \scomment{is there supposed to be something else here? this sentence isn't qualitative analysis}

% \begin{figure}
%     \centering
%     \includegraphics[width=2.5in]{images/workerplot.pdf}
%     \caption{Number of judged items per crowdworker compared to MACE's inferred ``proficiency'' estimates (a measure of reliability or accuracy).
%     \label{fig:workerplot}
%     }
% \end{figure}

\ignore{

\textbf{Annotator modeling: MACE} \label{sec:mace}
\noindent
We noticed a wide variation in how different workers approached the annotation task.  Since the task has substantial subjectivity, we hoped to better model which annotators were more reliable, in order to derive higher quality, aggregated labels for each item. Following \citet{Paun2018Comparing}, who found that MACE~\cite{hovy2013learning} was among several top-performing models to efficiently aggregate crowd-sourced NLP annotations, we apply the open source MACE software\footnote{\url{https://github.com/dirkhovy/MACE}} with default settings to the dataset of judgments on both test and non-test items.\footnote{We used MACE in purely unsupervised mode in order to better explore errors or disagreements between annotators and our putative gold standard, as FigureEight's quality control system already ensures all annotators had at least 80\% agreement with the test items' labels.
\bto{relax this stmt if we don't end up analyzing it}} MACE is an unsupervised, joint probabilistic model of annotators and judgments for crowd-sourced settings which infers probabilistic labels for each annotated item weighted by the estimated proficiency of each annotator. 

% \begin{table}[]\centering
% \caption{Conditional confusion matrix for each label, calculated using raw item judgments. \bto{3 sigdigs \ag{what is meant by sigdigs?}}}
% \label{tab:cmm}
% \scriptsize
% \begin{tabular}{lrrrrr}\toprule
% &Pos &Neg &Uu &NE \\\midrule
% Pos &0.8777438 &0.007772895 &0.04166648 &0.07281682 \\
% Neg &0.03348749 &0.804026098 &0.03990946 &0.12257696 \\
% Uu &0.0722116 &0.016054478 &0.78684371 &0.12489021 \\
% NE &0.01222109 &0.004775154 &0.01209446 &0.9709093 \\
% Margins &0.12874304 &0.029882987 &0.07428542 &0.76708855 \\
% \bottomrule
% \end{tabular}
% \end{table}

% Figure~\ref{fig:workerplot} shows one point per crowdworker, plotting the number of annotations they provided (for non-test items), against their proficiencies, as estimated by MACE.  Like many crowd-sourced data collection settings, we had a small number of workers who supplied a very large number of labels (e.g.\ thousands), though there were many who supplied moderate and useful numbers of labels (e.g.\ dozens to hundreds).  Proficiency also varied widely, despite quality control heuristics. FigureEight's and our further quality control heuristics.
% While the most prolific annotators are not the most accurate, in general there is no correlation between these factors
% (Spearman $\rho=0.0002$).  The advantage of MACE, like other annotator models, is that 
% marginally informative judgments 
% from lower-quality annotators can still be used to help infer aggregate labels.

% > source("workerplot.r")
% > cor(ww$n,ww$comp,method='spearman')
%[1] 0.0002290604

MACE also infers posterior entropies for each item which can be used as an approximation for the model’s confidence in the prediction, lower entropy implies higher confidence~\cite{hovy2013learning}. We use these entropies to identify items with higher annotator disagreements. Table~\ref{table:disagreement} (Appendix) provides some of the difficult examples from our dataset where annotators had high disagreements. Most often, annotators find it difficult to disambiguate a positive/negative versus uncommitted factuality stance. \scomment{this is strange---shouldn't it be straightforward to disambiguate decidedly positive/negative items from uncommitted ones?} For instance, consider the following sentence with ``Author'' as source (marked in red) and ``good'' as event (marked in blue). 

\emph{\textcolor{red}{Author:} But when the crisis part actually involves putting us out of work , it 's hard to see how pride in our identity will do us any \textcolor{blue}{good}.}

For this example, 2 annotators voted positive, 1 voted negative and 2 voted for uncommitted class. The counter-factual nature of this statement probably confused the annotators. 

%\ag{how to argue about non-epistemic class?}

}



==> files/Experiments.tex <==
% !TEX root = ../main.tex
\section{Experiments}
\label{sec:experiments}

%in fine-tuning for the respective prediction task.

%\bto{XXX I COMMENTED THIS OUT, IT WAS APPEARING FOR SOME REASON}
%jack knife style predictions from cross validation {we assemble predictions from each of our dataset by concatenating predictions from each of the three folds. This ensures we don't loose information due to how averaging works over non linear metrics such as F1. Unification of testset bootstrapping for estimating confidence intervals which allows us to directly compare between multi domain and single domain settings.}

% \subsection{Model Training} \label{sec:modeltrain}
% We explored two settings for BERT-model training of all our models, including the source/event identification models and the epistemic stance classifier. (1) \textbf{Fine-Tuned \bert}:~We start with pre-trained \bert, updating both the task-specific layer and all \bert parameters in fine-tuning for the respective prediction task. (2) \textbf{Frozen \bert}: since the training sets are small, we try to reduce the number of learned parameters by using fixed \bert contextual embeddings, only updating the task-specific linear layer~\cite{peters-etal-2019-tune}.\ag{we perhaps don't need frozen models now; we experimented with them because PoliBelief was small, FactBank has decent size}


\begin{table*}[t]
\centering \scriptsize
\begin{tabular}{lrrrrrrrr}
\hline
\textbf{Model} &
  \multicolumn{1}{c}{\textbf{CT+}} &
  \multicolumn{1}{c}{\textbf{CT-}} &
  \multicolumn{1}{c}{\textbf{PR+}} &
  \multicolumn{1}{c}{\textbf{PS+}} &
  \multicolumn{1}{c}{\textbf{Uu}} &
  \multicolumn{1}{c}{\textbf{NE}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Macro Avg\\ (Non-NE)\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Macro Avg\\ (All)\end{tabular}}} \\ \hline
DeFacto~\cite{sauri2012you}            & 85.0 & 75.0 & 46.0 & 59.0  & 75.0 & -    & 70.0 & -    \\
SVM~\cite{sauri2012you, prabhakaran2010automatic}                & 90.0 & 61.0 & 29.0 & 39.0  & 66.0 & -    & 59.0 & -    \\
BiLSTM~\cite{qian-2018-gan}             & 85.2 & 74.0 & 58.2 & 61.3  & 73.3 & -    & 70.4 & -    \\
AC-GAN~\cite{qian-2018-gan}              & 85.5 & 74.1 & 63.1 & 65.4  & 75.1 & -    & 72.6 & -    \\
BERT~\cite{jiang2021thinks}     & 89.7 & 69.8 & 45.0 & 46.7 & 82.8 & 97.9 & 66.8 & 72.0 \\
RoBERTa (this work) & 90.7 & 78.4 & 51.4 & 62.7 & 84.8 & 97.8 & 73.6 & 77.6 \\ \hline
\end{tabular}
\caption{F1 scores for our RoBERTa based epistemic stance classifier and all baseline models.}
\label{tab:classifier_results}
\end{table*}

% RoBERTa (frozen)    &      &      &      &       &      &      &      &      \\

% BERT (frozen)       &      &      &      &       &      &      &      &      \\



% \ag{experiments with other models needs to be included, RoBERTa, BART and T5. Why? To demonstrate usefulness of this data due to domain shift.}

\subsection{Performance} 
\paragraph{Source and Event Identification Models}
Our source and event identification models achieve a macro-averaged F1 score of $81.8\pm0.019$ and $85.78\pm 0.007$, respectively, slightly improving upon the only existing prior work of ~\citet{qian-2018-gan} by $1.85\%$ and $1.29\%$ respectively, with pairwise significance tests resulting in $p$-values less than $0.01$. We also experimented with a joint model to identify sources and events; however, individual classifiers gave us better performance. 
% See Appendix~\ref{sec:appendix_model_performance} for more detailed comparisons and error analysis.  

\paragraph{Epistemic Stance Classifier}
% Table~\ref{tab:classifier_results} shows the performance of our epistemic stance classifier. 
We compare our model against several baselines, including rule-based methods (DeFacto;~\citet{sauri2012you}), machine learning classifiers (SVM developed by \citet{sauri2012you} using lexico-syntactic features proposed by \citet{prabhakaran2010automatic}), and neural network based methods (BiLSTM and AC-GAN developed by \citet{qian-2018-gan}) as described in \S\ref{sec:existing_models}.\footnote{Since the DeFacto implementation is not available, we compare our model's predictions on the FactBank test set against evaluation statistics derived from the test set confusion matrix reported by \citeauthor{sauri2012you}. We use implementation provided at \url{https://github.com/qz011/ef_ac_gan} for SVM, BiLSTM and  AC-GAN baselines.}
% \bto{which models did we implement or use and where did the implementations come from if so? is it the case all except DeFacto were models YOU ran? you merely state ``we compare'' which does not make this clear.} \ag{added the url of implementation in footnote}
% \ag{does the last sentence make it clearer? I mainly used the git repo provided in \citet{qian-2018-gan}}
We also extend the author-only BERT model developed by \citet{jiang2021thinks} to support multi-source predictions in line with our modeling approach. 

% for an author-only continuous valued stance prediction model. For fair comparisons with our model, we instead train the \bert model for multi-class classification task and extend it for multi-source predictions in line with our modeling approach. In particular, we compare against following baselines.

% \textbf{\defacto}: a foundational rule-based multi-source system \cite{sauri2012you} that uses manually developed context polarity lexicons for predicates and modal particles in a recursive constituency tree analysis algorithm. 
% % Since the DeFacto implementation is not available,\footnote{\emph{Citation redacted for anonymity}} we compare our model's predictions on the FactBank test set against evaluation statistics derived from the test set confusion matrix reported by \citeauthor{sauri2012you}.
% \textbf{SVM}~\cite{sauri2012you}: a multi-source model using word-level lexical features (e.g., word's POS tag, lemma, verb type etc), and dependency tree based syntactic features proposed by ~\citet{prabhakaran2010automatic}. 
% \textbf{BiLSTM}~\cite{qian-2018-gan} model encoding dependency parse tree based structural features (e.g., dependency path between a source and SIP)  and architecturally more complex \textbf{GAN}-based model~\cite{qian-2018-gan}, where a generator generates syntactic features conditioned on stance labels and discriminator determines whether the features are generated. The GAN model also consists of auxiliary classification task to determine the final epistemic stance label. \textbf{BERT} ~\cite{jiang2021thinks}: an author-only continuous valued stance prediction model. For fair comparisons with our model, we instead train the \bert model for multi-class classification task and extend it for multi-source predictions in line with our modeling approach. \ag{there is some repetition between this para and the ``existing models" section (section 2), is there a way to discuss it at one place only?}

Table~\ref{tab:classifier_results} shows the performance of our RoBERTa based epistemic stance classifier and comparisons with above mentioned baselines. The RoBERTa model performs the best obtaining a macro-averaged F1 score of $77.6\pm$0.011 on all six epistemic labels and an F1 score of $73.6\pm$0.031 on the original five epistemic labels (excluding the \nonepistemic label). Although the RoBERTa model has a much simpler architecture, it performs the same or better than AC-GAN. All pairwise significance tests resulted in $p$-values less than $0.01$.

% BTO: commented out 7/1 3:15pm
%A more detailed error analysis on the correlation between model performance and presence of negative polarity items, is provided in Appendix~\ref{sec:appendix_stance_classifier}. 

% \paragraph{Error Analysis: Negative Polarity Items}
% The \emph{CT-} class is the most rare in \factbank, and it is useful to identify for a possible future use case of finding disagreements in text.  For corpus exploration, an alternative to our model could be to simply view sentences with
% explicit negative polarity items (NPIs); such sentences\footnote{Using an NPI list of: 
% \emph{no}, \emph{not}, \emph{n't},
% \emph{never}, \emph{nobody}, \emph{none} } indeed contain a large majority (88.2$\%$) of \factbank's gold standard \emph{CT-} tuples. They are still uncommon within NPI-containing sentences (13.5$\%$ of such tuples are \emph{CT-}),
% and quite rare within sentences without NPIs (0.33$\%$ of such tuples are \emph{CT-}).
% For this challenging CT- class, the model attains a F1 score of 78.4$\%$. To examine the model performance on CT- class in political domain, we qualitatively analyzed correct classifications. We observe that the model exhibits ability to deal with complex connections between negation-bearing constructions like \emph{Unable to}, \emph{refuse}, etc. (Table \ref{tab:npi_examples}).


% \subsection{Error Analysis: Negative Polarity Items}
% The \emph{CT-} class is the most rare in \factbank, and it is useful to identify for a possible future use case of finding disagreements in text.  For corpus exploration, an alternative to our model could be to simply view sentences with
% explicit negative polarity items (NPIs); such sentences\footnote{Using an NPI list of: 
% \emph{no}, \emph{not}, \emph{n't},
% \emph{never}, \emph{nobody}, \emph{none} } indeed contain a large majority (88.2$\%$) of \factbank's gold standard \emph{CT-} tuples. They are still uncommon within NPI-containing sentences (13.5$\%$ of such tuples are \emph{CT-}),
% and quite rare within sentences without NPIs (0.33$\%$ of such tuples are \emph{CT-}).
% For this challenging CT- class, the model attains a F1 score of 78.4$\%$. To examine the model performance on CT- class in political domain, we qualitatively analyzed correct classifications. We observe that the model exhibits ability to deal with complex connections between negation-bearing constructions like \emph{Unable to}, \emph{refuse}, etc. (Table \ref{tab:npi_examples}).

\ignore{
\subsection{Evaluation on Political Opinion Domain}
\label{sec:pb_results}
Our epistemic stance classifier is trained on \factbank, a dataset specific to the news domain. However, before using this model for political discourse analysis, we must ensure that the model performs well under domain shift. Thus, we evaluate our epistemic stance classifier on \polibelief; an evaluation dataset which we explicitly crowdsource in the political opinion domain. We next describe our data collection process followed by model performance on this dataset.

\paragraph{\polibelief Corpus Description:}
We collect a simplified evaluation dataset specific to the political domain by drawing sentences from Contemporary American Ideological Books (CAIB; \citet{sim2013measuring}), a corpus of mass-market political nonfiction books in English authored by U.S. politicians, media activists, and opinion elites with diverse ideological perspectives. To reduce the annotator burden and simplify the annotation task, we heuristically pre-identify sources and events. Unlike FactBank's criteria of using SIPs that may miss some relevant sources and events annotated in TimeBank and AQUAINT TimeML\footnote{\url{https://web.archive.org/web/20070721130754/http://www.timeml.org/site/publications/specs.html}} that consider only short-term stative events of ``focal interest" in newswires, we use a loose and automatic filter to identify sources and events. We consider all nouns and pronouns as a source and identify all heads of sentential clauses as events. More details are provided in Appendix \S\ref{sec:appendix_polibelief}. 

% We collect crowdsourced epistemic stance annotations for sentences drawn from Contemporary American Ideological Books (CAIB; \citet{sim2013measuring}), a curated corpus of mass-market political nonfiction books in English authored by U.S. politicians, media activists, and opinion elites with diverse ideological perspectives. We heuristically pre-identify sources and events to ease annotator burden and simply the task. For source identification, a natural extension would be to use \factbank's SIP lexicons. However, such an approach could miss potentially relevant sources.\footnote{For example, Congress in ``Yesterday, \textbf{[Congress]$_{s}$} passed the bill to increase taxes." is not a source in \factbank since ``passed'' is not an SIP; however, it is reasonable to assess its epistemic stances toward bill passage and tax increases.} We instead use a simple and loose automatic filter that considers all nouns and pronouns as a source. To pre-identify events, again \factbank's approach of using events annotated in \timebank and AQUAINT TimeML\footnote{\url{https://web.archive.org/web/20070721130754/http://www.timeml.org/site/publications/specs.html}} has its own limitations, allowing only short-term stative events of ``focal interest" in newswires. Instead, we use Universal Dependencies parser\footnote{UD v1.3 \cite{NIVRE16.348} from CoreNLP 3.8.0's \texttt{english\_UD} model \cite{manning-etal-2014-stanford}} to identify all heads of sentential clauses, as a relatively loose but not totally unrestricted filter. See Appendix XX for more details.

% While identifying sources, we realized that \factbank's SIP-based approach for source identification could miss potentially relevant sources.\footnote{For example, Congress in ``Yesterday, \textbf{[Congress]$_{s}$} passed the bill to increase taxes." is not a source in \factbank since ``passed'' is not an SIP; however, it is reasonable to assess its epistemic stances toward bill passage and tax increases.} We instead use a simple and loose automatic filter that considers all nouns and pronouns as a source (and excludes ones with a noun or adjective parent, in order to restrict to the head word of a noun phrase). The special \emph{Author} source is additionally included.
% Finally, we additionally simplify from \factbank by not considering nested sources,\footnote{For any non-author source, we define their epistemic stance as what the author depicts it as. \factbank allows more complex nesting, such as an author's depiction of one source's view of another source.}to facilitate simple training of crowdworker annotators.

% Again for event identification, \factbank's approach of using events annotated in \timebank and AQUAINT TimeML\footnote{\url{https://web.archive.org/web/20070721130754/http://www.timeml.org/site/publications/specs.html}} has its own limitations. We find that while TimeBank's (and thus FactBank's) semantic criteria
% for event identification \cite{timebankcorpus} consider states to be events, 
% they only include ones with a short enough temporal duration to be of ``focal interest'' in newswire text,
% thus excluding, for example, ``New York is on the east coast.''
% But for epistemic stance prediction, especially in ideological texts, these predicates can be of great interest. Thus, we identify all heads of sentential clauses as events, as a relatively loose but not totally unrestricted filter. Using a Universal Dependencies parser,\footnote{UD v1.3 \cite{NIVRE16.348} from CoreNLP 3.8.0's \texttt{english\_UD} model \cite{manning-etal-2014-stanford}} we designate the tree's
% root as an event, as well as its descendants connected via any of the relations \emph{acl:relcl, advcl, ccomp, csubj, parataxis, xcomp}.\footnote{This heuristic has the limitation of excluding nominal events, such as \emph{The \underline{firing}$_{e}$ of the manager}, which introduce more complications to identify; they are left for future work.}

We next collect stance annotations for a full cross product of all identified sources and events. We adopt a simplified three-class coarse view of the more fine-grained \factbank's annotations or the continuous annotations sometimes collected in previous work~\cite{stanovsky2017integrating}. We chose this approach due to ease of annotation, since \citet{de-marneffe-etal-2012-happen} found that many of the disagreements in their annotations were about degree of confidence (e.g., certain vs. probable vs. possible), and \citet{hobby-2000-communication} also found the distinction between possible and probable was hard to make in the biomedical domain.\footnote{Note that even with a coarse three-class discrete model, \citet{stanovsky2017integrating}-style continuous-valued output can be produced through probabilistic predictions.\ag{reword it}}

In particular, we do not distinguish between various degrees of expressed uncertainty, instead grouping all such cases\footnote{PR+, PS+, Uu} into \emph{Uncommitted} (Uu). In addition, we include \emph{Positive} (Pos) and \emph{Negative} (Neg) classes as parallels for CT+ and CT- categories in \factbank. Finally, we also include the \emph{Non-Epistemic} (NE) stance when it does not make sense to assess an epistemic stance for a given source-event pair. This category account for any spurious event-source pairs that may result from the overgeneration of sources and events. See Appendix~\ref{sec:appendix_polibelief} for more details on stance definitions. 


% \begin{enumerate*}
%     \item \textbf{\emph{Positive} (Pos)}: According to the source, the event definitely happened, or the described proposition is true. 
%     \item \textbf{\emph{Negative} (Neg)}: According to the source, the event definitely did not happen, or the described proposition is false.
%     \item \textbf{\emph{Uncommitted} (Uu)}: The source is unsure about the status of the event, is trying to stay uncommitted whether the event happened, or is reporting someone else's beliefs.
%     \item \textbf{\emph{Non-Epistemic} (NE)}: It does not make sense to assess an epistemic stance for this source-event pair.\footnote{This was defined for annotators as: ``Answer N/A if the question doesn't make sense; this includes questions where the highlighted source isn't something or someone that holds beliefs, either in general or in the context of this specific question.''} This category account for any spurious event-source pairs that may result from the overgeneration of sources and events. 
% \end{enumerate*}

% The three epistemic classes described above are a coarse view of the more fine-grained \factbank's annotations or the continuous annotations sometimes collected in previous work~\cite{stanovsky2017integrating}---we do not distinguish between various degrees of expressed uncertainty, instead grouping all such cases into \emph{Uncommitted}. We chose this approach due to ease of annotation,
% since \citet{de-marneffe-etal-2012-happen} found that many of the disagreements in their annotations were about degree of confidence (e.g., certain vs. probable vs. possible), and \citet{hobby-2000-communication} also found the distinction between possible and probable was hard to make in the biomedical domain.\footnote{Note that even with a coarse three-class discrete model, \citet{stanovsky2017integrating}-style continuous-valued output can be produced through probabilistic predictions.}

\begin{table}
\centering \small
%\begin{tabular}{c|ccccc}
%\hline \addlinespace[0.05cm]
%\multirow{2}{*}{\#Sentences} & \multicolumn{5}{c}{\#Tuples}    \\ \addlinespace[0.05cm] \cline{2-6}  \addlinespace[0.05cm]
\begin{tabular}{cccc|c}
 Pos  & Neg & Uu  & NE   & Total \\ \addlinespace[0.05cm] \hline \addlinespace[0.05cm]
1176 & 254 & 641 & 6394 & 8465  %\\ \addlinespace[0.05cm] \hline \addlinespace[0.05cm]
\end{tabular}
\caption{Counts for \emph{Positive}, \emph{Negative}, \emph{Uncommitted}, and \nonepistemic tuples in \polibelief.
\label{table:stats}}
\end{table}

\paragraph{Annotation Details}
%\jhg{This duplicates what I'm writing in 3.1, so we can probably drop or shorten this.}
For collecting epistemic stance annotations, we sampled one sentence from each of 308 books to ensure broad corpus diversity. (The 308 consisted of all books in an earlier version of CAIB.)  We did not attempt to filter to political discussion. To ensure a dataset with a range of complex linguistic and rhetorical phenomena, we considered sentences with more than 15 tokens and at least one embedded event.
%(see Events and Sources below).
% \jhg{Did you do any filtering to get sentences that involved political rhetoric? Or did you randomly choose a single sentence without any filtering or chance for rejection (e.g. if sentence were simply the author recalling trips to Lake Erie as a child).}
Annotations were collected on the Figure Eight platform. A prompt with pre-identified source and event is shown to the annotator and is asked to annotate epistemic stance for this event-source pair. A sample prompt is included on the dataset website. We obtain a raw inter-annotator agreement rate $0.793$ and chance-adjusted agreement rate (Krippendorff $\alpha$) $0.554$ for 51,805 annotations. This is broadly in line with reported chance-adjusted agreement rates in prior literature (see Appendix~\ref{sec:appendix_polibelief} for more detailed comparisons). 

Finally, to infer aggregated labels we use the MACE model and software \cite{hovy2013learning},\footnote{\url{https://github.com/dirkhovy/MACE}}
which uses Bayesian unsupervised learning to weigh the judgments of different annotators by their relative reliability;
\citet{Paun2018Comparing} found MACE was one of the best models for crowdsourced annotation aggregation. We use the most probable label inferred by MACE as the final label.\footnote{We experimented with MACE's item-level posteriors for soft label training \cite{fornaciari-etal-2021-beyond}, but observed similar results as training on hard labels.} After quality filtering, our dataset consists of 8465 annotated event-source pairs spanning 308 sentences from the CAIB corpus (Table~\ref{table:stats}). Additional Details of our initial pilot study, annotator details, payment rates and data filtering procedures can be found in Appendix~\ref{sec:appendix_polibelief}. 

% \paragraph{Our findings from the annotation study}
% While crowdsourcing \polibelief, we came across several challenges and important observations that can be useful for the research community while designing their own annotation efforts. 

% As mentioned before the agreement rate for this and related datasets is slightly lower than some of the conventional standards seen in NLP. A detailed qualitative analysis of examples highlighted the genuine and substantive ambiguity of this task (Table XX in Appendix). As part of future work, we recommend modelling stances as a distribution of annotator responses \cite{pavlick2019inherent}, rather than forcing into a single answer. 
% \ag{need to mention some more challenges found}

\paragraph{Model Evaluation on \polibelief}
We next describe the evaluation of our epistemic stance classifier (trained on \factbank) on \polibelief dataset. Since the epistemic stance classifier trained on \factbank predicts one of the six fine-grained stance categories and \polibelief has coarse-grained annotations with four categories, we map \factbank's epistemic stances to \polibelief's coarser categories.\footnote{FactBank's certain-positive and certain-negative classes (CT+, CT-) are mapped to \emph{Positive} and \emph{Negative} classes in \polibelief respectively; all others, that express any degree of uncertainty, are combined to \emph{Uncommitted}. This mapping also results in class prevalence close to that of \polibelief corpus.} The model achieves a macro F1 score of 51.6$\%\pm 0.008$, which is XXX \ag{what do we compare this performance with?, how do we know what is the baseline on this dataset?} In addition, we conducted a manual evaluation of model predictions to identify cases where the model made genuine errors versus cases where noise/genuine ambiguity in annotations made it hard to interpret the correct label (details provided in Appendix~\ref{sec:appendix_manual_polibelief}). Based on our human evaluation, the model achieves an F1 score of XX$\%$, signifying that the model performs reasonable under domain shift and can be used for political discourse analysis. \ag{manual analysis of model predictions is one way i could think of justifying that evaluation under domain shift was successful. Is there any other way we can argue?}

\paragraph{Lessons Learnt from \polibelief}
\ag{this section again is one way i could think of bringing in polibelief's discussion. Looking forward to more comments or other ways to talk about model evaluation on \polibelief}
We next describe the challenges and key lessons we learnt while crowdsourcing epistemic stance annotations and using these annotations for model development. Our observations demonstrates that annotating epistemic stances is indeed a complex linguistic task and obtaining high quality data comparable to expert annotations is difficult.

\begin{enumerate}[leftmargin=*]
    \item[] \textbf{Genuine Ambiguity in Annotations}: We conducted a manual analysis of crowdsourced annotations in \polibelief, observing genuine ambiguity in annotations (Table~\ref{tab:polibelief_ambiguity}). We found that annotators often conflated the notion of a source that can potentially hold beliefs with the subject of a sentence, sometimes marking spurious entities as holding stances/beliefs. For instance, in Table~\ref{tab:polibelief_ambiguity}A, [dollar]$_{s}$ and [nation]$_{s}$, subject of the respective sentences, are marked as having Pos/Uu stance for most events by majority annotators, however their beliefs are not expressed in the sentence. We also observed genuine ambiguity over future tense events with some annotators marking the event with Pos stance, while others marking those events with Uu stance. In Table~\ref{tab:polibelief_ambiguity}B, three annotators marked Uu, and two annotators marked Pos stances for \underline{continue}$_{e}$ and \underline{become}$_{e}$ events). We also observed instances of annotation noise, the stance annotations for coreferent sources (e.g., \emph{author} and the first-person pronouns such as I, we, us, etc.) didn't agree for a given event. For instance, in Table~\ref{tab:polibelief_ambiguity}C, while most annotators mark (Author, figure, Uu); they also mark (I, figure, NE); even though [Author]$_{s}$ and [I]$_{s}$ are coreferent and ideally should have same stances. In some cases, annotators relied on a false heuristic, marking every event positionally appearing before the source in a given sentence with NE stance. All of these observations indicate the high linguistic complexity of this task and challenges in crowdsourcing epistemic stances. \ag{a possible cross-question: why not collect new set of annotations after revising guidelines to account for these observed issues?}
    
    % Annotators often marked the same stances for the \textit{author} source and first-person plural pronouns (e.g., we, us, etc.) mentioned in a given sentence, unifying the distinctions between a group's stance versus the author's own stance.
    
    % Our \nonepistemic category captured two notions, spurious source-event pairs and valid sources but with no epistemic stances expressed in the given sentence.
    
    \item[] \textbf{Model over-fitting when trained on \polibelief}: We also conducted experiments where we used \polibelief as a training dataset, by sequentially fine-tuning \bert model on \factbank followed by \polibelief. This approach of sequential fine-tuning has been shown effective in various domain adaptation and low resource settings~\cite{pruksachatkun-etal-2020-intermediate, vu-etal-2020-exploring, han-eisenstein-2019-unsupervised}. The sequentially fine-tuned model achieved an F1 score of 67.2$\%\pm$0.016, which is better than the model trained only on \factbank (51.6$\%\pm 0.008$; See Appenidx~\ref{sec:appendix_model_performance_polibelief} for additional results). However, on manual analysis of predictions, we observe that the model over-fits to annotation noise and idiosyncrasies of the \polibelief dataset. Based on these observations, we decided not to use \polibelief for training purposes. However, our manual analysis provided us with a good sense of model performance under domain shift, giving us the confidence to use this model for political discourse analysis.
\end{enumerate}

\ag{I wasn't able to fit many of the previous experimental results, as they were all based on models trained on \polibelief, or error analysis on \polibelief dataset. Currently they have been moved to Appendix. Open to suggestions on bringing back some experiments or planning new ones which fit the context better.}


\begin{table*}[!htp]\centering
\scriptsize
\begin{tabular}{p{0.97\linewidth}}\toprule
A. Subject as a source with epistemic stances \\
$\bullet$ Author:~This means that we should expect that the \textbf{[dollar]$_{s}$} will \textbf{\underline{continue}$^{(1,0,2,1)}_{e}$} to be overvalued for some time to come. \\ 
$\bullet$ Author:~Our \textbf{[nation]$_{s}$} will \textbf{\underline{become}$^{(2,0,3,0)}_{e}$} a tarnished example and weaker in the eyes of the world. \\ \vspace{0.01} \hline \vspace{0.01}
B. Disagreement over future tense \\ 
$\bullet$ \textbf{[Author]$_{s}$}:~This means that we should expect that the dollar will \textbf{\underline{continue}$^{(2,0,3,0)}_{e}$} to be overvalued for some time to come. \\
$\bullet$ \textbf{[Author]$_{s}$}:~Our nation will \textbf{\underline{become}$^{(2,0,3,0)}_{e}$} a tarnished example and weaker in the eyes of the world. \\ \vspace{0.01} \hline \vspace{0.01}
C. Annotation Noise \\ \vspace{0.05}
$\bullet$ \textbf{[Author]$_{s}$}:~I told Elaine that I wouldn't leave Garden Spires until we could \textbf{\underline{figure}$^{(1,0,3,1)}_{e}$} something out. \\
$\bullet$ Author:~I told Elaine that \textbf{[I]$_{s}$} wouldn't leave Garden Spires until we could \textbf{\underline{figure}$^{(0,0,1,5)}_{e}$} something out. \\ \vspace{0.01}

$\bullet$ \textbf{[Author]$_{s}$}: If this is \textbf{\underline{passed,}$^{(0,0,5,0)}_{e}$} we are going to see our budget deficit increase, according to the Congressional Budget Office. \\
$\bullet$ Author: If this is \textbf{\underline{passed,}$^{(1,0,1,3)}_{e}$} \textbf{[we]$_{s}$} are going to see our budget deficit increase, according to the Congressional Budget Office.
\bottomrule
\end{tabular}
\caption{Examples of genuine ambiguity and annotation noise in \polibelief; sources are highlighted in bold, events are underlined, with number of (positive, negative, uncommitted, non-epistemic) stance annotations.}\label{tab:polibelief_ambiguity}
\end{table*}

}

% We also conducted experiments where we used \polibelief as training dataset, by sequentially fine-tuning \bert model on \factbank followed by \polibelief. This approach of sequential fine-tuning has been shown effective in various domain adaptation and low resource settings~\cite{pruksachatkun-etal-2020-intermediate, vu-etal-2020-exploring, han-eisenstein-2019-unsupervised}. We evaluated this model on jackknifed predictions on the entire \polibelief (constructed from concatenation of each test fold, from the three different cross-validation models),
% which also allows for consistent statistical testing and comparisons among different models. The sequentially fine-tuned model achieved an F1 score of 67.2$\%\pm$0.016, which is better than the model trained only on \factbank (47.1$\%\pm$xx). However, on manual analysis of predictions, we observe that the model over-fits to annotation noise in the \polibelief dataset. Thus, we do not recommend using \polibelief for model training. \ag{to myself: write properly that \polibelief is crowdsourced and has genuine ambiguity in its annotations. Moreover, given the complexity of this linguistic task, it is hard to collect a high quality dataset in crowdsource settings and thus has higher annotation noise. Since the size of \polibelief is small and it has annotation noise, model possibly over fits to idiosyncrasies of this dataset. Thus, we do not recommend using \polibelief for training purposes. It can however, gives a sense of model performance under domain shift.}  

% \paragraph{Performance}
% Figure~\ref{fig:ablation} shows the performance of the model variants on PoliBelief. Fine-tuning consistently outperforms frozen embeddings. In-domain training (PB) outperforms solely out-of-domain training (FB), indicating substantial domain shift in the data. The performance is best when combining both training sets (FB+PB) in the sequential fine-tuning setup, successfully leveraging the out-of-domain FactBank data, greatly improving the difficult \emph{Negative} class performance similar to the other epistemic classes (Table \ref{tab:detailedPoli}). 

% BTO i just cut this
% \textcolor{red}{In this paper, we assess the significance of all our results by considering the variability associated with the finite test set, following the traditional practices. However, recent work has observed variability due to instability of \bert fine-tuning on small datasets ~\cite{dodge-jesse-etal-2020-fine}. We conduct an analysis to explore these two sources of variability in our results. To compute variability due to the finite test set, we find variance across many bootstrap samples, where, for each bootstrap sample, we average the performance over five different model restarts. To compute the variability due to training, we calculate the average variance in model performance over bootstrap samples. Note that the sum of these two variabilities is equal to the variance obtained due to a random selection of bootstrap sample and model restart due to the law of total variance.}

% \textcolor{red}{
% We find that the variance due to model training dominates the total variance. Further, comparing the in-domain fine-tuning with the sequential fine-tuning setup, we observe that sequential fine-tuning results in reduced total variance. While the variance due to the finite test set is similar for both the models  ($\sim 6\times10^{-5}$), the variance due to model training is significantly higher for the model trained with in-domain data \bto{is this supposed to be 10 to -5?} (PB; $28.1 \times 10^{-4}$) than the sequentially fine-tuned model (FB+PB; $8.2 \times 10^{-5}$). We hypothesize that this reduced variance is due to the availability of more training data in the sequential fine-tuned setup. We leave a deeper investigation of these findings and the relation between the above two source of statistical variability in NLP models for future work.}
% BTO END comment-out 10/14


% \textcolor{red}{Given the recent work~\cite{dodge-jesse-etal-2020-fine} on instability of \bert fine-tuning on small datasets, we examine the robustness of our model to training stability. We investigate two sources of variability 1) variance due to model training owing to random restarts of the model 2) variance due to a finite sample of the test dataset.}


% \textcolor{red}{Comparing the in-domain fine-tuning with the sequential fine-tuning setup, we observe that sequential fine-tuning results in reduced total variance. While the variance due to the finite test set is similar for both the models ($\sim$ $6\times10^{-5}$), the variance due to model training is significantly higher for the model trained with in-domain data (PB; $28.1 \times 10^{-4}$) than the sequentially fine-tuned model (FB+PB; $8.2 \times 10^{-5}$). We hypothesize that this reduced variance is due to the availability of more training data in the sequential fine-tuned setup. We leave its validation for future work.}

% The sequential fine-tuning setup also helps improve the model training stability.

% \textcolor{red}{
% However, the model with in-domain training (PB) comes close to the performance of the sequentially fine-tuned model (FB+PB). We conducted a bootstrapping-based one-sided hypothesis test~\cite{berg-kirkpatrick-etal-2012-empirical} to examine the statistical significance of the difference between these two models. We use the difference in the macro-averaged F1 score of two models as our statistic (T); with the null hypothesis that the two models perform equivalently ($H_{0}: T = 0$ and $H_{1}: T \neq 0$) — the test results in a p-value of 0.16, which is not strong evidence against the null hypothesis at level 0.05 (alpha). A pairwise significance test for all other model combinations resulted in strong evidence against the null hypothesis at 0.05 level.
% }

% \textcolor{red}{Although the performance gain of the sequentially fine-tuned model is not statistically significant w.r.t performance of model fine-tuned on in-domain data (PB), sequential fine-tuning helps improve the model training stability. We examined the variance breakdown of the two models in terms of 1 variance due to model training (owing to random restarts of the model) 2 variance due to a finite sample of the test dataset. While the variance due to the finite test set is similar for both the models (~$6\times10^{-05}$), the variance due to model training is an order magnitude higher for the model trained with in-domain data (PB; $2.8 \times 10^{-04}$) than the sequentially fine-tuned model (FB+PB; $8.2 \times 10^{-05}$). We hypothesize that reduced variance can be explained by the availability of more training data in the sequential fine-tuned setup. We leave detailed validation for future work.}

%: the performance of pre-trained language models---such as \bert---can be improved by further training the model on a data-rich domain before fine-tuning it on a target domain. 

% The model obtains the best results with fine-tuned \bert model using the multi-domain setting (training on \factbank and \polibelief sequentially). The model performance improves by fine-tuning in contrast with the frozen \bert setting for both single-domain and multi-domain training setup.  

%Comparing the single-domain fine-tuned model on \polibelief with the multi-domain fine-tuned model, we observe that transferring from \factbank improves the macro-average F1 score and also helps improve the F1 of the \emph{Negative} class, which is the rarest and most challenging class.

% \begin{figure}[t]
% \includegraphics[width=\linewidth]{images/model_results_CI.pdf}
% \caption{BERT PoliBelief performance (with 95$\%$ CI) under different training and model settings
% PB (\polibelief) and FB (\factbank) refer to the training dataset; FB and FB+PB are domain adaptation settings (\S\ref{sec:modeltrain}--\ref{sec:pb_results}). All pairwise significance tests give $p$-values less than 0.01.
% %Frozen and Fine-Tune refers to the model setting. All models are evaluated on \polibelief with average results reported over three-fold cross validation.
% }
% \label{fig:ablation}
% \end{figure}

%Finally, comparing the single-domain fine-tuned model in \factbank versus the model fine-tuned in \polibelief shows that the model's performance degrades ($16.8\%$ absolute F1), indicating a significant domain shift and the need for an annotated resource specific to the political domain.


% \begin{table}[!htp]\centering
% \caption{Performance of \bert model evaluated on PoliBelief corpus.}\label{tab:detailedPoli}
% \small
% \begin{tabular}{lrrrr}\toprule
% \multirow{2}{*}{\textbf{Label}} &\multirow{2}{*}{\textbf{Precision}} &\multirow{2}{*}{\textbf{Recall}} &\multirow{2}{*}{\textbf{F1}} \\
% & & & \\\midrule
% Pos &0.6319 &0.6873 &0.6561 \\
% Neg &0.5449 &0.6556 &0.5919 \\
% Uu &0.5157 &0.5160 &0.5107 \\
% NE &0.9383 &0.9119 &0.9248 \\
% \multirow{2}{*}{\textbf{Macro Avg}} &\multirow{2}{*}{0.6577} &\multirow{2}{*}{0.6927} &\multirow{2}{*}{0.6709} \\
% & & & \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[!htp]
% \centering \small
% \begin{tabular}{lccc}
% \hline
% Label      & Precision & Recall & F1              \\ \hline
% Pos        & 63.2\scriptsize{$\pm$0.024}      & 68.7\scriptsize{$\pm$0.023}   & 65.8\scriptsize{$\pm$0.012} \\
% Neg        & 54.5\scriptsize{$\pm$0.053}      & 65.6\scriptsize{$\pm$0.055}   & 59.7\scriptsize{$\pm$0.047} \\
% Uu         & 51.6\scriptsize{$\pm$0.036}      & 51.6\scriptsize{$\pm$0.035}   & 51.1\scriptsize{$\pm$0.031} \\
% NE         & 93.8\scriptsize{$\pm$0.005}      & 91.2\scriptsize{$\pm$0.006}   & 92.5\scriptsize{$\pm$0.004} \\ \addlinespace[0.2cm]
% Macro Avg. & 65.8\scriptsize{$\pm$0.017}      & 69.3\scriptsize{$\pm$0.017}   & 67.2\scriptsize{$\pm$0.016} \\ \hline
% \end{tabular}
% \caption{Performance (with 95$\%$ CI) of the multi-domain (FB+PB) fine-tuned BERT model on PoliBelief (\S\ref{sec:pb_results}).}\label{tab:detailedPoli}
% \end{table}

% \begin{table}[!htp]
% \centering \small
% \begin{tabular}{lccc}
% \hline
% Label     & Precision & Recall & F1   \\ \hline
% Pos       & 63.2     & 68.7   & 65.8 $\pm$ 0.010 \\
% Neg       & 54.5      & 65.6   & 59.7$\pm$0.024 \\
% Uu        & 51.6     & 51.6   & 51.1$\pm$0.016 \\
% NE        & 93.8      & 91.2   & 92.5$\pm$0.002 \\ \addlinespace[0.2cm]
% Macro Avg. & 65.8      & 69.3   & 67.2+0.008 \\ \hline
% \end{tabular}
% \caption{Performance of the multi-domain (FB+PB) fine-tuned BERT model on PoliBelief (\S\ref{sec:pb_results}).}\label{tab:detailedPoli}
% \end{table}

%\vspace{-0.35cm}
% %%Table for Comparison to DeFacto
% \begin{table}[tbh]
% \centering \small
% \begin{tabular}{lcccc}
% \hline \addlinespace[0.05cm]
% Model & Pos  & Neg  & Uu   & Macro Avg. \\ \addlinespace[0.05cm] \hline \addlinespace[0.15cm]
% DeFacto               & \scriptsize{84.0} & \scriptsize{75.0} & \scriptsize{76.0} & \scriptsize{78.3}       \\
% BERT                   & \scriptsize{90.3$\pm$ .006} & \scriptsize{77.0$\pm$ .045} & \scriptsize{85.6$\pm$ .008} & \scriptsize{84.2$\pm$ .016}      \\ \addlinespace[0.05cm] \hline 
% \end{tabular}
% \caption{F1 measure for epistemic-only three-class models evaluated on \factbank (\S\ref{sec:defacto}).}
% \label{tab:bert_defacto}
% \end{table}


% \begin{table}[tbh]
% \centering \small
% \begin{tabular}{lcc}
% \hline
% Label      & DeFacto & BERT                         \\ \hline
% Pos        & 84.0    & 90.3\scriptsize{$\pm$0.011} \\
% Neg        & 75.0    & 77.0\scriptsize{$\pm$0.088} \\
% Uu         & 76.0    & 85.6\scriptsize{$\pm$0.015} \\ \addlinespace[0.05cm]
% Macro Avg. & 78.3    & 84.2\scriptsize{$\pm$0.031} \\ \hline
% \end{tabular}
% \caption{F1 measure for epistemic-only three-class models evaluated on \factbank (\S\ref{sec:defacto}).}
% \label{tab:bert_defacto}
% \end{table}


% \begin{table*}[!htp]\centering
% \scriptsize
% \begin{tabular}{p{0.8\linewidth}}\toprule
% $\bullet$ \textbf{[Author]$_{s}$:}  Unable to \textbf{\underline{reach}$_{e}$} Russo in the era before cell phones, the House Speaker, Jim Wright, kept the vote open for some twenty minutes while an aide coaxed a member to change his vote to yes. \\
% $\bullet$ Author: \textbf{[John Boehner]$_{s}$}, the Speaker of the House, refused to \textbf{\underline{address}$_{e}$} immigration reform in 2013. \\
% $\bullet$ \textbf{[Author]$_{s}$:}  That logic obviously failed to \textbf{\underline{impress}$_{e}$} the Supreme Court eighty-six years later when it decided that corporations are people under the First Amendment, entitled to hire as many lobbyist adventurers as they can possibly afford. \\
% $\bullet$ \textbf{[Author]$_{s}$:}  These White House scandals are truly becoming as much of a scandal for the national media that refuses to hold the government and this White House \textbf{\underline{accountable}$_{e}$}. \\
% $\bullet$ Author: \textbf{[People]$_{s}$} are beginning to move worlds apart and find it increasingly difficult to \textbf{\underline{establish}$_{e}$} common ground. \\
% $\bullet$ \textbf{[Author]$_{s}$:}  When those intentions turned into actions , President Obama consistently failed to \textbf{\underline{take}$_{e}$} any meaningful steps to stop him. \\
% $\bullet$ \textbf{[Author]$_{s}$:}  Although still incapable of actually \textbf{\underline{cutting}$_{e}$} spending, except for needed defense, conservative leaders imply our national crisis is merely some budgeting blunder remediable through a balanced budget amendment to the Constitution. \\
% \bottomrule
% \end{tabular}
% \caption{Samples without NPI correctly predicted by BERT Model from PoliBelief Corpus; sources are highlighted in red, events are highlighted in blue.}\label{tab:npi_examples}
% \end{table*}

% \subsection{Comparison to DeFacto} \label{sec:defacto}
% To test just the model itself,
% we evaluate only on the FactBank dataset,
% comparing a single-domain model to the foundational \defacto
% multi-source system \cite{sauri2012you}. DeFacto is a rule-based method, 
% based on manually developed context polarity lexicons for predicates and modal particles, which are used in a recursive constituency tree analysis algorithm.
% It produces one of eight fine-grained epistemic stance classes for certain event-source pairs in a sentence.
%  of  that is trained on eight fine-grained classes, namely factual, probable, possible, not possible, not probable, counterfactual, uncertain, and certain but unknown output. 
% Since the DeFacto implementation is not available,\footnote{\emph{Citation redacted for anonymity}}
% we compare our model's predictions on the FactBank test set against evaluation statistics derived from the test set confusion matrix reported by \citeauthor{sauri2012you}, by mapping FactBank's epistemic stances to our coarser categories.\footnote{DeFacto/FactBank's certain-positive and certain-negative classes (CT+, CT-) are mapped to our \emph{Positive} and \emph{Negative} classes respectively; all others, that express any degree of uncertainty, are combined to \emph{Uncommitted}. This mapping also results in class prevalence close to that of \polibelief corpus.} 
%\bto{any other justif? does prevalence match polibelief's?}}
%With these new classes, we collapse the reported \defacto's confusion matrix on \factbank data and present it in Table~\ref{tab:defacto_confusion} (See Appendix). 

% Since \factbank consists only of event-source pairs manually annotated for epistemic stances,
% it does not include any \nonepistemic stances, and DeFacto does not produce them.
% To fairly compare to DeFacto, we evaluate the performance of a separate \bert model trained (fine-tuned) on \factbank's training set and evaluated on its test set, for a three-class classification task.
% % Consequently, we examine the performance of the \bert model fine-tuned for a three-class classification task
% % to fairly compare to DeFacto. \bto{train split? new model?} 
% Validating our approach, the \bert model outperforms \defacto in this setting for all categories ($p=0.04$, two-tailed test), 
% though the \emph{Negative} class is only slightly improved (Table~\ref{tab:bert_defacto}). 
%\textcolor{red}{Two-sided pairwise significance test for \bert and \defacto model resulted in a p-value of 0.04, rejecting the null hypothesis of equivalent model performances.} 

% \begin{table}[!htp]\centering
% \caption{Comparison of \bert model and \defacto on \factbank corpus.}\label{tab:bert_defacto}
% \small
% \begin{tabular}{lcccc}\toprule
% \textbf{Model} &\textbf{Macro Avg.} &\textbf{Pos} &\textbf{Neg} &\textbf{Uu} \\\midrule
% DeFacto &78.3 &84.0 &75.0 &76.0 \\
% BERT &84.2 &90.3 &77.0 &85.6 \\
% \bottomrule
% \end{tabular}
% \end{table}



% \bto{All results tables should be multiplied by 100 and rounded to closest 3 significant digits (1 decimal point), e.g. "67.1". do this with a script not manually (if you have to do manual, use truncation not rounding to avoid human error, but be consistent everywhere)}






% %% Table for NPI (Qualitative Analysis of Model) 
% \begin{table*}[!htp]\centering
% \scriptsize
% \begin{tabular}{p{0.97\linewidth}}\toprule
% $\bullet$ \textbf{[Author]$_{s}$}:~Unable to \textbf{\underline{reach}$_{e}$} Russo in the era before cell phones, the House Speaker, Jim Wright, kept the vote open for some twenty minutes while an aide coaxed a member to change his vote to yes. \\
% $\bullet$ Author:~\textbf{[John Boehner]$_{s}$},~the Speaker of the House, refused to \textbf{\underline{address}$_{e}$} immigration reform in 2013. \\
% $\bullet$ Author:~\textbf{[People]$_{s}$} are beginning to move worlds apart and find it increasingly difficult to~\textbf{\underline{establish}$_{e}$}~common ground. \\
% $\bullet$ \textbf{[Author]$_{s}$}:~Although still incapable of actually \textbf{\underline{cutting}$_{e}$}~spending, except for needed defense, conservative leaders imply our national crisis is merely some budgeting blunder remediable through a balanced budget amendment to the Constitution. \\
% \bottomrule
% \end{tabular}
% \caption{Examples of \emph{CT-} epistemic stances, in sentences without explicit NPIs in \polibelief, that BERT correctly predicts; sources are highlighted in bold, and events are underlined.}\label{tab:npi_examples}
% \end{table*}


%In addition to domain differences, there are linguistic differences between \factbank and \polibelief, which may affect model performance on these two datasets. Unlike \factbank, \polibelief has a lower (higher) percentage of instances with explicit (implicit) negations: 82.23$\%$ (88.23$\%$) of negative class tuples from \polibelief (\factbank) contain explicit mention of negative polarity items (NPIs).\footnote{We consider words such as:  as explicit mentions of NPIs.} As a result, the \polibelief corpus offers more instances with implicit negations, which are more challenging for models to predict but also more interesting. Table~\ref{tab:detailedPoli} summarizes the detailed performance of the multi-domain fine-tuned \bert model on the \polibelief corpus, illustrating that the model finds it hard to predict the tuples from negative class. Furthermore, Table~\ref{tab:npi_poli} mentions the performance metrics (F1) of the model over instances with/without explicit mention of NPIs. The observations from the Table~\ref{tab:npi_poli} are in accordance with results noted in~\citet{rudinger2018neural} and \citet{jiang2021thinks} for other neural models of epistemic stance prediction: 
%\begin{enumerate*}[label=(\arabic*)]
%\item It is difficult for the model to predict instances with implicit negations, accounting for reduced negative-class F1 when NPIs are implicitly mentioned (40$\%$) compared to explicit negation (63$\%$).
%\item The NPI mentions lead the model to predict negative class even when the label is positive, accounting for lower positive-class F1 when NPIs are explicitly mentioned (60$\%$) compared to implicit negation (68$\%$).~Similar observation is true for uncommitted class.
%\end{enumerate*} 
%Table~\ref{tab:npi_examples} mentions some of the difficult instances with negative epistemic stance and with implicit negations from the \polibelief corpus that the \bert model can identify correctly. 

% 36.15$\%$ (15.31$\%$) of  all tuples in \polibelief (\factbank) have negative polarity items(NPIs) in their respective sentences. Furthermore, 

% \begin{table}[]
% \centering
% \caption{NPI analysis on PoliBelief Data using Two Stage Fine-Tuned BERT model, 82.23$\%$ of negative tuples have NPI in the sentence.
% 36.15$\%$ of all tuples have NPI in the sentence. \ag{I think F1 score and Gold Class prevalence is sufficient from this table?}}
% \label{tab:npi_poli}
% \scriptsize
% \npdecimalsign{.}
% \nprounddigits{2}
% \begin{tabular}{|n{3}{3}|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{} & \textbf{Pos} & \textbf{Neg} & \textbf{Uu} & \textbf{NE} \\ \hline
% \multicolumn{1}{|l|}{} & \multicolumn{4}{c|}{\textbf{Recall}} \\ \hline
% NPI & 0.646465 & 0.718593 & 0.410891 & 0.913554 \\ \hline
% Without NPI & 0.727772 & 0.348837 & 0.557647 & 0.917774 \\ \hline
% \multicolumn{1}{|l|}{} & \multicolumn{4}{c|}{\textbf{Precision}} \\ \hline
% NPI & 0.57485 & 0.576613 & 0.458564 & 0.939172 \\ \hline
% Without NPI & 0.651917 & 0.483871 & 0.553738 & 0.940227 \\ \hline
% \multicolumn{1}{|l|}{} & \multicolumn{4}{c|}{\textbf{F1}} \\ \hline
% NPI & 0.608558 & 0.639821 & 0.43342 & 0.926186 \\ \hline
% Without NPI & 0.687759 & 0.405405 & 0.555686 & 0.928865 \\ \hline
% \multicolumn{1}{|l|}{} & \multicolumn{4}{c|}{\textbf{Gold Class Prevalence}} \\ \hline
% NPI & 0.096397 & 0.064589 & 0.065563 & 0.77345 \\ \hline
% Without NPI & 0.167432 & 0.007903 & 0.078111 & 0.746554 \\ \hline
% \end{tabular}
% \npnoround
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \tiny
% \begin{tabular}{lrrrr|rrrr}
% \hline \addlinespace[0.05cm]
% \multicolumn{1}{l}{\multirow{2}{*}{}} & \multicolumn{4}{c|}{NPI}             & \multicolumn{4}{c}{Without NPI}       \\ \addlinespace[0.05cm]\cline{2-9} \addlinespace[0.05cm]
% \multicolumn{1}{l}{}                  & {Prec.}   & {Rec.}    & {F1}      & {Prev.}  & {Prec.}   & {Rec.}    & {F1}      & {Prev.}   \\ \addlinespace[0.05cm] \cline{2-9} \addlinespace[0.05cm]
% Pos                                   & 57.5  & 64.6 & 60.9 & 9.6 & 65.2 & 72.8 & 68.8 & 16.7 \\
% Neg                                   & 57.7 & 71.9 & 64.0 & 6.5 & 48.4 & 34.9 & 40.5 & 0.8  \\
% Uu                                    & 45.9 & 41.1 & 43.3  & 6.6 & 55.4 & 55.8 & 55.6 & 7.8  \\
% NE                                    & 93.9 & 91.4 & 92.6 & 77.3 & 94.0 & 91.8 & 92.9 & 74.7 \\ \addlinespace[0.05cm] \hline
% \end{tabular}
% \caption{NPI analysis on \polibelief corpus using multi-domain fine-tuned \bert model. \emph{Prev.} denotes the gold class prevalence for each class based on the estimates by MACE. \emph{Prec.}, \emph{Rec.} and \emph{F1} denotes the precision, recall and F1 measure respectively for each class. \ag{I think F1 score and Gold Class prevalence is sufficient from this table?}}
% \label{tab:npi_poli}
% \end{table}

%% Table for NPI (Quantitative Analysis of Model) 
%\begin{table}[]
%\centering
%\begin{tabular}{lrr|rr}
%\hline
%\multirow{2}{*}{} & \multicolumn{2}{c|}{NPI} & \multicolumn{2}{c}{~Without~NPI~}  \\ \addlinespace[0.05cm] \cline{2-5}  \addlinespace[0.05cm]
%                 & F1        & Prev.   & F1            & Prev.      \\ \addlinespace[0.05cm] \hline \addlinespace[0.05cm]
%Pos                                   & 60.9   & 9.6       & 68.8       & 16.7         \\
%Neg                                   & 64.0   & 6.5       & 40.5       & 0.8         \\
%Uu                                    & 43.3    & 6.6       & 55.6       & 7.8          \\
%NE                                    & 92.6   & 77.3       & 92.9       & 74.7         \\ \addlinespace[0.05cm] \hline
%\end{tabular}
%\caption{NPI analysis on \polibelief using multi-domain fine-tuned \bert model. \emph{Prev.} denotes the class prevalence for each class in \polibelief based on MACE estimates.}
%\label{tab:npi_poli}
%\end{table}
%

%% NPI

==> files/Hedging.tex <==
% !TEX root = ../main.tex
\section{Case Study: Hedging and power}
\label{sec:hedging}
% \bto{i introduced term `hedging' in title. is there a reason you avoid it here?}
% \ag{i just think by using the term "hedging" one may ask why not use a hedge word list?} \ag{we can call it hedging and should we add something like this "While hedging and hesitations have been utilized to measure lack of commitment~\cite{philips1985william}, political discourse can feature many more strategies beyond a simple lexicon, such as indirect speech acts, hypothetical if-then clauses, or framing claims as questions~\cite{fraser2010hedging}. Thus, analyzing hedging requires understanding of syntactic contexts within which claims are expressed, making our epistemic stance framework suitable for such analysis."}
\noindent
\citet{jalilifar2011power} examine the relationship between an author's perceived political power and their expressed commitment to their beliefs.
% and the commitment of the author to their beliefs,
%as expressed in sociopolitical interactions, for various political actors. 
While hedging and hesitations have been utilized to measure lack of commitment~\cite{philips1985william}, political discourse can feature many more strategies beyond a simple lexicon of hedge words, such as indirect speech acts, hypothetical if-then clauses, or framing claims as questions~\cite{fraser2010hedging}. Thus, analyzing hedging requires understanding of syntactic contexts within which claims are expressed, which our model can tackle. We establish the external validity of our proposed epistemic stance framework by computationally replicating the findings of \citet{jalilifar2011power}'s manual content analysis. To ensure the external validity of our proposed epistemic stance framework, we  computationally replicate the findings of \citet{jalilifar2011power}'s manual content analysis (See Appendix~\ref{}.

% In this section, we establish an external validity of our proposed epistemic stance framework by computationally replicating an existing political case study~\citet{jalilifar2011power}. The study examines the relationship between author commitment (expressed in socio-political interactions such as political speeches or interviews) and the their perceived political power, i.e, are actors with greater (perceived) political power more likely to express a stronger commitment to their beliefs when communicating with their audience? While hedging and hesitations have been utilized to measure lack of commitment~\cite{philips1985william}, political discourse can feature many more strategies beyond a hedge word list, such as indirect speech acts, hypothetical if-then clauses, or framing claims as questions~\cite{fraser2010hedging}. Thus, analyzing the author's commitment level requires understanding of syntactic contexts within which claims are expressed, making our epistemic stance framework suitable for such analysis.

% Our first case study computationally examines the relationship between author commitment level and their political power using our epistemic stance classifier, also establishing an external validity to the proposed framework. Specifically, we want to investigate whether the commitment authors express towards their beliefs in socio-political interactions (e.g., political speeches or interviews) is correlated with their perceived political power. 

% Prior socio-linguistic studies use hedges and hesitations~\cite{philips1985william} as measures of lack of commitment. However, political discourse can feature many more strategies beyond a hedge word list to express lack of commitment~\cite{fraser2010hedging}. For instance, actors may use indirect speech acts, frame claims as questions or express their beliefs using hypothetical if-then clause constructions, all displaying lack of commitments. Thus, in our study, we analyze different belief commitments expressed by authors using epistemic stance framework that takes into account the syntactic contexts within which propositions are expressed. 

The study examines transcripts of topically similar television interviews of three political figures,
George W.\ Bush (at the time, incumbent U.S.\ president), 
Jimmy Carter (former U.S.\ president),
 and David Coltart (founding member of Zimbabwe’s main opposition party).\footnote{Authors also analyzed interviews by U.S.\ politician Sarah Palin, but we these transcripts were not available at the provided URL.} %All designations reported at the time of interview. The authors also analyzed interviews by Sarah Palin, an American politician, however, her transcripts are not accessible via the links provided in the paper.}
% (at the time of writing this manuscript)} 
% Each of these interviews was carefully selected to ensure that the topic of discussion was similar and that they all happened around a similar time. 
For each interview transcript, we employ our epistemic stance classifier to predict the stance of the political figure (author source) towards all extracted events,
and 
calculate each author's uncertainty level as the fraction of events with a \emph{PR+} or \emph{PS+} epistemic stance.
% \footnote{Note that while the number of analyzed interviews are small, the total number of tuples analyzed is much larger for each politician.\ag{ADD Number}} 

%(over all utterances by a politician)

% \bto{I'm confused what we replicated. Did we get the same ordering of the 3 figures? Please say so directly if so. The following is ambiguous esp since the power interp of coltart vs carter is weird.}\ag{yes, we got the same ordering, adding a sentence}
We find the same ordering of commitment as the previous work:
Bush using the fewest uncertain \textit{PR+/PS+} stances ($5.41\%$),
with progressively more for Carter ($8.32\%$) and Coltart ($12.2\%$).
This follows \citeauthor{jalilifar2011power}'s interpretation of commitment being correlated to power (Bush being the highest status, for example).

%we also observe an inverse relationship between political power and author commitment to their beliefs within these three examples. 
%Bush, being the current president and thus highest status, displays the least use of uncertain \textit{PR+/PS+} stances ($5.41\%$). Carter uses more uncertainty ($8.32\%$), and Coltart the most ($12.2\%$). Although in power, Coltart expressed lesser commitment levels than the retired \textit{Jimmy Carter}, possibly due to his party's internal political volatility~\}.
% More detailed qualitative examples are provided in Appendix XX.


%% BTO: no no no the point is the old paragraph, by leading with the interp, confuses readers who doubt their interp! their interp is bad.
%% \ag{Similar to the manual analysis, our computational model predicts the same order among the three politicians when ranked by their commitment levels.} 
%% \bto{yes though make the whole paragarph not repetitive and cleaner}\ag{reworded}

% For instance, he resorts to a series of hedges and shows lack of precise knowledge in order to shield himself from any adverse consequences.

% Although in power, he expressed lesser commitment levels than the retired \textit{Jimmy Carter}.~\citet{jalilifar2011power} attributes this observation to his party's internal political volatility.


==> files/Limitations.tex <==
% !TEX root = ../main.tex
\section{Limitations}
Footing shift can be analyzed further with multi-modal data, such as facial expressions etc.

Coreference is not perfect in our analysis. 



% In this paper, I discuss footing both in general and with reference to the analysis of paralinguistic clues in one of Hillary Clinton's electoral speeches. I try to show that footing is a construction that can be obtained through textual strategies, while shifts of footing are often signalled through facial expression. It is impossible to analyse the notion of footing without taking into account the oral dimension of communication. I also propose that one should look at the interplay of the argu- mentative structure and of shifts of footing.

